Cosmic evolution of supermassive black holes: A view into the next two decades

The discoveries made over the past 20 years by Chandra and XMM-Newton surveys in conjunction with multiwavelength imaging and spectroscopic data available in the same fields have significantly changed the view of the supermassive black hole (SMBH) and galaxy connection. These discoveries have opened up several exciting questions that are beyond the capabilities of current X-ray telescopes and will need to be addressed by observatories in the next two decades. As new observatories peer into the early Universe, we will begin to understand the physics and demographics of SMBH infancy (at $z>6$) and investigate the influence of their accretion on the formation of the first galaxies ($\S$ 2.1). We will also be able to understand the accretion and evolution over the cosmic history (at $z\sim$1-6) of the full population of black holes in galaxies, including low accretion rate, heavily obscured AGNs at luminosities beyond the reach of current X-ray surveys ($\S$2.2 and $\S$2.3), enabling us to resolve the connection between SMBH growth and their environment.

==> WP_author_lists_final.tex <==
%     
Francesca Civano $^{1}$,   
Nico Cappelluti $^{2}$,   
Ryan Hickox $^{3}$,   
Rebecca Canning $^{4,5}$,   
%     
James Aird $^{6}$,   
Marco Ajello $^{7}$,   
Steve Allen $^{4,5}$,   
Eduardo Ba\~nados $^{8}$,   
Laura Blecha $^{9}$,   
William N. Brandt $^{10}$,  
Marcella Brusa $^{11}$,   
Francisco Carrera $^{12}$,   
Massimo Cappi $^{13}$,   
Andrea Comastri $^{13}$,   
Klaus Dolag $^{14,15}$,   
Megan Donahue $^{16}$,   
Martin Elvis $^{1}$,   
Giuseppina Fabbiano $^{1}$,   
Francesca Fornasini $^{1}$,   
Poshak Gandhi $^{17}$,   
Antonis Georgakakis $^{18}$,   
Kelly Holley-Bockelmann $^{19}$,   
Anton Koekemoer $^{20}$,   
Andrew Goulding $^{21}$,   
Mackenzie Jones $^{1}$,   
Sibasish Laha $^{22}$,   
Stephanie LaMassa $^{20}$,   
Giorgio Lanzuisi $^{13}$,   
Lauranne Lanz $^{3}$,   
Adam Mantz $^{4,5}$,   
Stefano Marchesi $^{7}$,   
Mar Mezcua $^{23}$,   
Beatriz Mingo $^{24}$,   
Kirpal Nandra $^{18}$,   
Daniel Stern $^{25,26}$,   
Doug Swartz $^{27}$,   
Grant Tremblay $^{1}$,   
Panayiotis Tzanavaris $^{28}$,   
Alexey Vikhlinin $^{1}$,   
Fabio Vito $^{29,30}$,   
Belinda Wilkes $^{1}$,   
%
Scott Anderson $^{31}$,   
Vallia Antoniou $^{1,32}$,   
Manuel Aravena $^{33}$,   
Ashraf Ayubinia $^{34}$,   
Mitchell Begelman $^{35}$,   
Arash Bodaghee $^{36}$,   
Tamara Bogdanovi\'c $^{37}$,   
Rozenn Boissay-Malaquin $^{38}$,   
Angela Bongiorno $^{39}$,   
Peter Boorman $^{17}$,   
Stefano Borgani $^{40}$,   
Richard Bower $^{41}$,   
Laura Brenneman $^{1}$,   
Volker Bromm $^{42}$,   
Esra Bulbul $^{1}$,   
David Burrows $^{10}$,   
Claude Canizares $^{43}$,   
Chien-Ting Chen $^{27}$,   
Igor V. Chilingarian $^{1}$,  
Damian J. Christian $^{44}$,  
Benedetta Ciardi $^{15}$,   
Alison Coil $^{22}$,   
Thomas Connor $^{45}$,   
Paolo Coppi $^{46}$,   
Darren Croton $^{47}$,   
Akaxia Cruz $^{31}$,   
Raffaele D\'Abrusco $^{1}$,   
Filippo D'Ammando $^{13}$,   
Romeel Dav\'e $^{48}$,   
Gisella De Rosa $^{20}$,  
Ivan Delvecchio $^{49}$,   
Casey DeRoo $^{50}$,   
Kelly A. Douglass $^{51}$,  
Abraham Falcone $^{10}$,   
Xiaohui Fan $^{52}$,   
Claude-Andr\'e Faucher-Gigu\`ere $^{53}$,   
Gary Ferland $^{54}$,   
K. E. Saavik Ford $^{55}$, 
William Forman $^{1}$,   
Antonella Fruscione $^{1}$,   
Keigo Fukumura $^{56}$,   
Massimiliano Galeazzi $^{2}$,   
David Garofalo $^{57}$,   
Massimo Gaspari $^{21}$,   
Lisseth Gavilan Marin $^{58}$,  
Jonathan Gelbord $^{59}$,   
Vittorio Ghirardini $^{1}$,   
Roberto Gilli $^{13}$,   
Omaira Gonz\'alez Mart\'in $^{60}$,  
Dale Graessle $^{1}$,   
Gian Luigi Granato $^{40}$,  
Paul J. Green $^{1}$,  
Richard Griffiths $^{61}$,   
Melanie Habouzit $^{62}$,   
Martin Haehnelt $^{63}$,   
Daryl Haggard $^{64}$,   
Nimish Hathi $^{20}$,   
Jeffrey Hazboun $^{65}$,   
Ralf K. Heilmann $^{43}$,  
Lars Hernquist $^{1}$,   
Julie Hlavacek-Larrondo $^{66}$,
Phil Hopkins $^{25}$,
David James $^{1}$,   
Manasvita Joshi $^{67}$,   
Philip Kaaret $^{50}$,   
Elias Kammoun $^{68}$,   
Nikita Kamraj $^{25}$,   
Margarita Karovska $^{1}$,   
Demosthenes Kazanas $^{28}$,   
Ildar Khabibullin $^{15,69}$,   
Dong-Woo Kim $^{1}$,   
Juna A. Kollmeier $^{45}$,  
Albert Kong $^{70}$,   
Alvaro Labiano $^{71}$,   
Claudia Lagos $^{72}$,   
George Lansbury $^{63}$,   
Erwin T. Lau $^{2}$,  
Denis Leahy $^{73}$,   
Bret Lehmer $^{74}$,   
Laura A. Lopez $^{75}$,  
Lorenzo Lovisari $^{1}$,   
Ray A. Lucas $^{20}$,  
Chelsea MacLeod $^{1}$,   
Kristin K. Madsen $^{25}$,  
W. Peter Maksym $^{1}$,  
Alberto Masini $^{3}$,   
Barry McKernan $^{55}$,   
Takamitsu Miyaji $^{76}$,   
Richard Mushotzky $^{77}$,   
Adam Myers $^{78}$,   
Qingling Ni $^{10}$,   
Joy Nichols $^{1}$,   
Kenichi Nishikawa $^{79}$,   
Emil Noordeh $^{4,5}$,   
Paul Nulsen $^{1}$,   
Anna Ogorzalek $^{4,5}$,
Feryal Ozel $^{52}$,
Fabio Pacucci $^{80}$,   
Frits Paerels $^{81}$,   
Antonella Palmese $^{82}$,   
Aaron B. Pearlman $^{25}$,  
Eric Perlman $^{83}$,   
Richard M. Plotkin $^{84}$,  
Stephanie Podjed $^{3}$,   
Meredith Powell $^{46}$,   
Francis A. Primini $^{1}$,  
Andrew Ptak $^{28}$,   
Mitchell Revalski $^{36}$,   
David Rosario $^{41}$,   
Bassem Sabra $^{85}$,   
Dhaka Sapkota $^{2}$,   
Gerrit Schellenberger $^{1}$,   
Dominic Sicilian $^{2}$,   
Lorenzo Sironi $^{81}$,   
Patrick Slane $^{1}$,   
Benny Trakhtenbrot $^{86}$,   
Virginia Trimble $^{87}$,   
Sara Turriziani $^{88}$,   
Reinout van Weeren $^{89}$,  
Cristian Vignali $^{11}$,   
Robert V. Wagoner $^{4,5}$,  
Devin Walker $^{3}$,   
Junxian Wang $^{34}$,   
Norbert Werner $^{90}$,   
Lacey West $^{74}$,   
J. Craig Wheeler $^{42}$,  
Daniel Wik $^{91}$,   
Benjamin Williams $^{31}$,   
Diana Worrall $^{92}$,   
Wei Yan $^{3}$,   
Guang Yang $^{10}$,

% %     
% Francesca Civano $^{1}$   
% Nico Cappelluti $^{2}$   
% Ryan Hickox $^{3}$   
% Rebecca Canning $^{4,5}$   
% %     
% James Aird $^{6}$   
% Marco Ajello $^{7}$   
% Steve Allen $^{4,5}$   
% Eduardo Ba\~nados $^{8}$   
% Laura Blecha $^{9}$   
% William N. Brandt $^{10}$  
% Marcella Brusa $^{11}$   
% Francisco Carrera $^{12}$   
% Massimo Cappi $^{13}$   
% Andrea Comastri $^{13}$   
% Klaus Dolag $^{14,15}$   
% Megan Donahue $^{16}$   
% Martin Elvis $^{1}$   
% Giuseppina Fabbiano $^{1}$   
% Francesca Fornasini $^{1}$   
% Poshak Gandhi $^{17}$   
% Antonis Georgakakis $^{18}$   
% Kelly Holley-Bockelmann $^{19}$   
% Anton Koekemoer $^{20}$   
% Andrew Goulding $^{21}$   
% Mackenzie Jones $^{1}$   
% Sibasish Laha $^{22}$   
% Stephanie LaMassa $^{20}$   
% Giorgio Lanzuisi $^{13}$   
% Lauranne Lanz $^{3}$   
% Adam Mantz $^{4,5}$   
% Stefano Marchesi $^{7}$   
% Mar Mezcua $^{12}$   
% Beatriz Mingo $^{23}$   
% Kirpal Nandra $^{18}$   
% Daniel Stern $^{24,25}$   
% Doug Swartz $^{26}$   
% Grant Tremblay $^{1}$   
% Panayiotis Tzanavaris $^{27}$   
% Alexey Vikhlinin $^{1}$   
% Fabio Vito $^{28,29}$   
% Belinda Wilkes $^{1}$   
% %     
% Scott Anderson $^{30}$   
% Vallia Antoniou $^{1,31}$   
% Manuel Aravena $^{32}$   
% Ashraf Ayubinia $^{33}$   
% Mitchell Begelman $^{34}$   
% Arash Bodaghee $^{35}$   
% Tamara Bogdanovi\'c $^{36}$   
% Rozenn Boissay-Malaquin $^{37}$   
% Angela Bongiorno $^{38}$   
% Peter Boorman $^{17}$   
% Stefano Borgani $^{39}$   
% Richard Bower $^{40}$   
% Laura Brenneman $^{1}$   
% Volker Bromm $^{41}$   
% Esra Bulbul $^{1}$   
% David Burrows $^{10}$   
% Claude Canizares $^{42}$   
% Chien-Ting Chen $^{26}$   
% Igor V. Chilingarian $^{1}$  
% Damian J. Christian $^{43}$  
% Benedetta Ciardi $^{15}$   
% Alison Coil $^{22}$   
% Thomas Connor $^{44}$   
% Paolo Coppi $^{45}$   
% Darren Croton $^{46}$   
% Akaxia Cruz $^{30}$   
% Raffaele D\'Abrusco $^{1}$   
% Filippo D'Ammando $^{13}$   
% Romeel Dav\'e $^{47}$   
% Gisella De Rosa $^{20}$  
% Ivan Delvecchio $^{48}$   
% Casey DeRoo $^{49}$   
% Kelly A. Douglass $^{50}$  
% Abraham Falcone $^{10}$   
% Xiaohui Fan $^{51}$   
% Claude-Andr\'e Faucher-Gigu\`ere $^{52}$   
% Gary Ferland $^{53}$   
% K. E. Saavik Ford $^{54}$ 
% William Forman $^{1}$   
% Antonella Fruscione $^{1}$   
% Keigo Fukumura $^{55}$   
% Massimiliano Galeazzi $^{2}$   
% David Garofalo $^{56}$   
% Massimo Gaspari $^{21}$   
% Lisseth Gavilan Marin $^{57}$  
% Jonathan Gelbord $^{58}$   
% Vittorio Ghirardini $^{1}$   
% Roberto Gilli $^{13}$   
% Omaira Gonz\'alez Mart\'in $^{59}$  
% Dale Graessle $^{1}$   
% Gian Luigi Granato $^{39}$  
% Paul J. Green $^{1}$  
% Richard Griffiths $^{60}$   
% Melanie Habouzit $^{61}$   
% Martin Haehnelt $^{62}$   
% Daryl Haggard $^{63}$   
% Nimish Hathi $^{20}$   
% Jeffrey Hazboun $^{30}$Bothell   
% Ralf K. Heilmann $^{42}$  
% Lars Hernquist $^{1}$   
% Julie Hlavacek-Larrondo $^{65}$   
% David James $^{1}$   
% Manasvita Joshi $^{66}$   
% Philip Kaaret $^{49}$   
% Elias Kammoun $^{67}$   
% Nikita Kamraj $^{24}$   
% Margarita Karovska $^{1}$   
% Demosthenes Kazanas $^{27}$   
% Ildar Khabibullin $^{15}$ $^{68}$  
% Dong-Woo Kim $^{1}$   
% Juna A. Kollmeier $^{44}$  
% Albert Kong $^{69}$   
% Alvaro Labiano $^{70}$   
% Claudia Lagos $^{71}$   
% George Lansbury $^{62}$   
% Erwin T. Lau $^{2}$  
% Denis Leahy $^{72}$   
% Bret Lehmer $^{73}$   
% Laura A. Lopez $^{74}$  
% Lorenzo Lovisari $^{1}$   
% Ray A. Lucas $^{20}$  
% Chelsea MacLeod $^{1}$   
% Kristin K. Madsen $^{24}$  
% W. Peter Maksym $^{1}$  
% Alberto Masini $^{3}$   
% Barry McKernan $^{54}$   
% Takamitsu Miyaji $^{75}$   
% Richard Mushotzky $^{76}$   
% Adam Myers $^{77}$   
% Qingling Ni $^{10}$   
% Joy Nichols $^{1}$   
% Kenichi Nishikawa $^{78}$   
% Emil Noordeh $^{4,5}$   
% Paul Nulsen $^{1}$   
% Anna Ogorzalek $^{4,5}$   
% Fabio Pacucci $^{79}$   
% Frits Paerels $^{80}$   
% Antonella Palmese $^{81}$   
% Aaron B. Pearlman $^{24}$  
% Eric Perlman $^{82}$   
% Richard M. Plotkin $^{83}$  
% Stephanie Podjed $^{3}$   
% Meredith Powell $^{45}$   
% Francis A. Primini $^{1}$  
% Andrew Ptak $^{27}$   
% Mitchell Revalski $^{35}$   
% David Rosario $^{40}$   
% Bassem Sabra $^{84}$   
% Dhaka Sapkota $^{2}$   
% Gerrit Schellenberger $^{1}$   
% Dominic Sicilian $^{2}$   
% Lorenzo Sironi $^{80}$   
% Patrick Slane $^{1}$   
% Benny Trakhtenbrot $^{85}$   
% Virginia Trimble $^{86}$   
% Sara Turriziani $^{87}$   
% Reinout van Weeren $^{88}$  
% Cristian Vignali $^{11}$   
% Robert V. Wagoner $^{4,5}$  
% Devin Walker $^{3}$   
% Junxian Wang $^{33}$   
% Norbert Werner $^{89}$   
% Lacey West $^{73}$   
% J. Craig Wheeler $^{41}$  
% Daniel Wik $^{90}$   
% Benjamin Williams $^{30}$   
% Diana Worrall $^{91}$   
% Wei Yan $^{3}$   
% Guang Yang $^{10}$   

